Formal Visual Modeling of Real-Time Systems in e-Motions: Two Case Studies

e-Motions is an Eclipse-based visual timed model transformation framework with a Real-Time Maude semantics that supports the usual Maude formal analysis methods, including simulation, reachability analysis, and LTL model checking. e-Motions is characterized by a novel and powerful set of constructs for expressing timed behaviors. In this paper we illustrate the use of these constructs --- and thereby implicitly investigate their suitability to define real-time systems in an intuitive way --- to define and formally analyze two prototypical and very different real-time systems: (i) a simple round trip time protocol for computing the time it takes a message to travel from one node to another, and back; and (ii) the EDF scheduling algorithm.

==> eptcsdata.tex <==
\providecommand{\firstpage}{49}
\providecommand{\publicationstatus}{Francisco Dur\'an and Vlad Rusu (Eds.):\\
Second International Workshop on Algebraic Methods\\
in Model-Based Software Engineering 2011 (AMMSE'11)\\
EPTCS 56, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.56.4}{10.4204/EPTCS.56.4}}
\pdfoutput=1

